AIR-Nets: An Attention-Based Framework for Locally Conditioned Implicit Representations

This paper introduces Attentive Implicit Representation Networks (AIR-Nets), a simple, but highly effective architecture for 3D reconstruction from point clouds. Since representing 3D shapes in a local and modular fashion increases generalization and reconstruction quality, AIR-Nets encode an input point cloud into a set of local latent vectors anchored in 3D space, which locally describe the object's geometry, as well as a global latent description, enforcing global consistency. Our model is the first grid-free, encoder-based approach that locally describes an implicit function. The vector attention mechanism from [Zhao et al. 2020] serves as main point cloud processing module, and allows for permutation invariance and translation equivariance. When queried with a 3D coordinate, our decoder gathers information from the global and nearby local latent vectors in order to predict an occupancy value. Experiments on the ShapeNet dataset show that AIR-Nets significantly outperform previous state-of-the-art encoder-based, implicit shape learning methods and especially dominate in the sparse setting. Furthermore, our model generalizes well to the FAUST dataset in a zero-shot setting. Finally, since AIR-Nets use a sparse latent representation and follow a simple operating scheme, the model offers several exiting avenues for future work. Our code is available at https://github.com/SimonGiebenhain/AIR-Nets.

==> figures/onetDataResultsTIKZ.tex <==
\begin{figure}[h!]
	\centering
	\begin{tikzpicture}
	\node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{AIR-Nets/figures/onetDataFinal_lowRes.png}};
	\node[above left = 0 and -2.7 of image] {Input};
	\node[above left = 0 and -8.4 of image] {\cite{if-net}};
	\node[above left = 0 and -11 of image] {Ours};
	\node[above left = 0 and -16 of image] {Ground Truth};
	\end{tikzpicture}
	\caption{\textbf{3D Reconstruction from Sparse Point Cloud:} The middle two column show a qualitative  comparison of IF-Nets proposed in \cite{if-net} and AIR-Nets. The input consisting of 300 points randomly sampled on the surface of the ground truth mesh and the ground truth are displayed in the left and right column respectively.}
	\label{pcRecSparse_fig}

\end{figure}

==> tables/recs_005_complete.tex <==
\begin{table*}[ht]
	\begin{center}
		\begin{tabular}{|r|c|c|c|c|c|c|} \hline
			&IoU$\uparrow$&$L_1\text{-Chamfer}\downarrow$ & $L_2\text{-Chamfer}\downarrow$ &Normal-Con.$\uparrow$&F-Score$\uparrow$&Val. Loss$\downarrow$ \\ \hline \hline
			%Input&-&-&0.0002& 0.00009&-&-&-&-\\ \hline
			$\text{ONet}_{300}$     & 0.755 &  8.41 & 31.09 & 0.891 & 0.797 & \\ 
			$\text{ConvONet}_{300}$ & 0.801 &  6.14 & 13.95 & 0.908 & 0.871 & \\ 
			$\text{IF-Net}_{300}$   & 0.763 &  6.97 & 16.22 & 0.895 & 0.84  & \\ 
			$\textbf{Ours}_{300}$   & 0.869 &  4.68 & 12.63 & 0.929  & 0.93 & \\
			 \hline
			$\text{ONet}_{3000}$    & 0.758 &  8.23 & 30.23 & 0.893 & 0.802 & \\ 
			$\text{ConvONet}_{3000}$& 0.888 &  3.97 &  5.6  & 0.935 & 0.953 & \\ 
			$\text{IF-Net}_{3000}$  & 0.924 &  3.03 &  2.14 & 0.951 & 0.985 &\\
			$\textbf{Ours}_{3000}$  & 0.925 &  3.28 &  7.4  & 0.952 & 0.978 & \\
			\hline
		\end{tabular}
	\end{center}
	\caption{}
	\label{tab:res_oData}
\end{table*}

==> tables/recs_nonoise_complete.tex <==
\begin{tabular}{|r|c|c|c|c|c|c|} \hline
			&IoU$\uparrow$&$L_1\text{-Chamfer}\downarrow$ & $L_2\text{-Chamfer}\downarrow$ &Normal-Con.$\uparrow$&F-Score$\uparrow$&Val. Loss$\downarrow$ \\ \hline \hline
			%Input&-&-&0.0002& 0.00009&-&-&-&-\\ \hline
			$\text{ONet}_{300}$     & 0.724 &  9.36 & 72.22 & 0.878 & 0.808 & \\ 
			$\text{ConvONet}_{300}$ & 0.723 &  8.42 & 45.32 & 0.876 & 0.841 & \\ 
			$\text{IF-Net}_{300}$   & 0.772 &  5.95 & 20.25 & 0.885 & 0.885 & \\ 
			$\textbf{Ours}_{300}$   & 0.913 &  3.24 &  5.32 & 0.95  & 0.964 & 0.075\\
			 \hline
			$\text{ONet}_{3000}$    & 0.704 & 10.02 & 72.59 & 0.874 & 0.786 & \\ 
			$\text{ConvONet}_{3000}$& 0.752 &  7.38 & 39.49 & 0.894 & 0.881 & \\ 
			$\text{IF-Net}_{3000}$  & 0.883 &  3.38 & 11.47 & 0.948 & 0.983 & \\
			$\textbf{Ours}_{3000}$  & 0.958 &  2.4  &  2.13 & 0.972 & 0.991 & 0.037\\
			\hline
\end{tabular}

==> tables/res_single_view.tex <==
\begin{tabular}{|c|l|c|c|c|c|} \hline
			&\multicolumn{1}{l|}{Model}&
			\multicolumn{1}{c|}{IoU$\uparrow$}&
			\multicolumn{1}{c|}{$L_1\text{-CD}\downarrow$}&
			\multicolumn{1}{c|}{\small{NC$\uparrow$}}&
			\multicolumn{1}{c|}{\small{F-Score$\uparrow$}} \\ \hline
			\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize{Sparse Input}}}}
            & \small{ONet}     &         0.647 &          0.01472 &         0.864 &           0.650\\ 
			& \small{ConvONet} &         0.693 &          0.01127 &         0.876 &           0.720\\ 
			& \small{IF-Net}   &         0.687 &          0.01223 &         0.873 &           0.710\\ 
			& \small{ours}     & \textbf{0.730}&  \textbf{0.00988}& \textbf{0.890}&   \textbf{0.764}\\
			 \hline
			 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize{Dense Input}}}}
			& \small{ONet}     &         0.616 &          0.01851 &         0.855 &           0.602\\ 
			& \small{ConvONet} &         0.731 &          0.00968 &         0.890 &           0.779\\ 
			& \small{IF-Net}   &         0.755 &          0.00947 &         0.900 &           0.799\\ 
			& \small{ours}  & \textbf{0.785}&  \textbf{0.00802}& \textbf{0.911}&   \textbf{0.836}\\
			\hline
\end{tabular}

==> tables/runtime.tex <==
\begin{tabular}{|c|l|c|c|c|c|c|c|} \hline
            &\multicolumn{1}{l|}{Model}&
            \multicolumn{1}{c|}{Training Speed}&
            \multicolumn{1}{c|}{Training Memory}&
            \multicolumn{1}{c|}{Inference Speed}&
            \multicolumn{1}{c|}{Opt. Epoch $\mathcal{D}_{A}$}&
            \multicolumn{1}{c|}{Opt. Epoch $\mathcal{D}_{B}$}\\ \hline
			\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize{Sparse Input}}}}
			 & \small{ONet}     &             0.0031 s/item &          0.13 GB/item &         2.0 s/mesh & 301 & 532\\ 
			 & \small{ConvONet} &             0.0023 s/item &          0.09 GB/item &         2.5 s/mesh &  65 & 499\\ 
			 & \small{IF-Net}   &             0.0465 s/item &          1.23 GB/item &         2.8 s/mesh &  10 &  43\\ 
			 & \small{$\text{Ours}_{M=50}$}&   0.0113 s/item &          0.33 GB/item &         3.1 s/mesh & 470 &  - \\ 
			 & \small{Ours}     &             0.0185 s/item &          0.57 GB/item &         3.1 s/mesh & 763 & 606\\ 
			\hline
			\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize{Dense Input}}}}
			 & \small{ONet}     &           0.0122 s/item &         0.31 GB/item &         1.9 s/mesh & 185 & 442\\ 
			 & \small{ConvONet} &           0.0027 s/item &         0.10 GB/item &         1.9 s/mesh &  47 & 345\\ 
			 & \small{IF-Net}   &           0.0465 s/item &         1.23 GB/item &         3.1 s/mesh &  27 & 140\\ 
			 & \small{$\text{Ours}_{M=50}$}& 0.0394 s/item &         0.53 GB/item &         2.8 s/mesh & 401 & - \\ 
			 & \small{Ours}     &           0.0421 s/item &         0.71 GB/item &         2.3 s/mesh & 468 & 296\\ 
			\hline
\end{tabular}

==> tables/setAbs.tex <==
\begin{tabular}{|c|l|c|c|c|c|} \hline
			&\multicolumn{1}{l|}{Model}&
			\multicolumn{1}{c|}{IoU$\uparrow$}&
			\multicolumn{1}{c|}{$L_1\text{-CD}\downarrow$}&
			\multicolumn{1}{c|}{\small{NC$\uparrow$}}&
			\multicolumn{1}{c|}{\small{F-Score$\uparrow$}} \\ \hline
			\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize{Sparse Input}}}}
			& \small{maxpool}      &         0.888 &          0.0037 &         0.940 &          0.952\\ 
			& \small{maxpool*}     &         0.893 &          0.0036 &         0.943 &          0.955\\ 
			& \small{singleStep}   &         0.891 &          0.0036 &         0.942 &          0.954\\ 
			& \small{ours}         & \textbf{0.896} & \textbf{0.0035}& \textbf{0.946}  & \textbf{0.957}\\
			 \hline
			 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize{Dense Input}}}}
			& \small{maxpool}    &         0.907 &            0.0040 &          0.946 &          0.965\\ 
			& \small{maxpool*}   &         0.905 &            0.0041 &          0.944 &          0.961\\ 
			& \small{singleStep} &         0.914 &            0.0034 &          0.949 &          0.969\\
			& \small{ours}       & \textbf{0.919} &   \textbf{0.0034} & \textbf{0.951} & \textbf{0.972}\\
			\hline
\end{tabular}

==> tables/single_view3000.tex <==
\begin{tabular}{|l|c|c|c|c|} \hline
			Model&
			{IoU$\uparrow$}&
			{$L_1\text{-CD}$$\downarrow$}&
			{\small{NC$\uparrow$}}&
			{\small{F-Score$\uparrow$}} \\ \hline
			 \small{ONet}     &         0.616 &          0.01851 &         0.855 &           0.602\\ 
			 \small{ConvONet} &         0.731 &          0.00968 &         0.890 &           0.779\\ 
			 \small{IF-Net}   &         0.755 &          0.00947 &         0.900 &           0.799\\ 
			 \small{ours}  & \textbf{0.785}&  \textbf{0.00802}& \textbf{0.911}&   \textbf{0.836}\\
			\hline
\end{tabular}

==> tables/test_equiv_DB.tex <==
\begin{tabular}{ c | c |} \hline
IoU & CD \\ 
 
    \begin{tabular}{l | c c c c c }
    model & None & trans & scale & rot & rotgrav \\ \hline
    ONet      & 0.680 & 0.135 & 0.548 & 0.210 & 0.491 \\
    ConvONet  & 0.824 & 0.644 & 0.735 & 0.452 & 0.723 \\
    IF-Net    & 0.908 & 0.839 & 0.871 & 0.866 & 0.898 \\
    Ours      & 0.924 & 0.858 & 0.897 & 0.868 & 0.908
    \end{tabular} 
& 
    \begin{tabular}{ c c c c c }
               None & trans & scale & rot & rotgrav \\ \hline
               0.0113 & 0.1104 & 0.0248 & 0.0606 & 0.0236 \\
               0.0054 & 0.0114 & 0.0080 & 0.0206 & 0.0084 \\
               0.0033 & 0.0052 & 0.0042 & 0.0044 &  0.0036\\
               0.0041 & x & x & x & x
    \end{tabular} 
\\ \hline
NC & F-Score \\ 
    \begin{tabular}{l | c c c c c }
    model & None & trans & scale & rot & rotgrav \\ \hline
    ONet      & 0.884 & 0.600 & 0.841 & 0.623 & 0.783 \\
    ConvONet  & 0.931 & 0.866 & 0.905 & 0.726 & 0.875 \\
    IF-Net    & 0.955 & 0.932 & 0.943 & 0.925 & 0.947 \\
    Ours      & 0.951 & 0.924 & 0.939 & 0.924 & 0.943
    \end{tabular} 
&
    \begin{tabular}{ c c c c c }
               None & trans & scale & rot & rotgrav \\ \hline
               0.0113 & 0.1104 & 0.0248 & 0.0606 & 0.0236 \\
               0.0054 & 0.0114 & 0.0080 & 0.0206 & 0.0084 \\
               0.983 & 0.935 & 0.961 & 0.945 & 0.975 \\
               0.969 & 0.931 & 0.952 & 0.928 & 0.969
    \end{tabular} 
\\ \hline
\end{tabular}
